Privacy Analysis of Samsung's Crowd-Sourced Bluetooth Location Tracking System

We present a detailed privacy analysis of Samsung's Offline Finding (OF) protocol, which is part of Samsung's Find My Mobile (FMM) location tracking system for locating Samsung mobile devices, such as Samsung smartphones and Bluetooth trackers (Galaxy SmartTags). The OF protocol uses Bluetooth Low Energy (BLE) to broadcast a unique beacon for a lost device. This beacon is then picked up by nearby Samsung phones or tablets (the {\em finder} devices), which then forward the unique beacon, along with the location it was detected at, to a Samsung managed server. The owner of a lost device can then query the server to locate their device. We examine several security and privacy related properties of the OF protocol and its implementation, from the perspectives of the owner, the finder and the vendor. These include examining: the possibility of identifying the owner of a device through the Bluetooth data obtained from the device, the possibility for a malicious actor to perform unwanted tracking against a person by exploiting the OF network, the possibility for the vendor to de-anonymise location reports to determine the locations of the owners or the finders of lost devices, and the possibility for an attacker to compromise the integrity of the location reports. Our findings suggest that there are privacy risks on all accounts, arising from issues in the design and the implementation of the OF protocol.

==> algorithms/command.tex <==
\begin{breakablealgorithm}
    \caption{The GATT command encryption/decryption algorithm} 
    \begin{algorithmic}[1]
         \STATE class MyClass:
         \STATE \hskip1.0em     def \_\_init\_\_(self, encryptionKey, nonce, cmd\_cnt):
         \STATE \hskip2.0em	        self.encryptionKey = encryptionKey
         \STATE \hskip2.0em	        self.nonce = nonce
         \STATE \hskip2.0em	        self.cmd\_cnt = cmd\_cnt
         \STATE \hskip2.0em	        self.key = self.getEncKey()
        \STATE
         \STATE \hskip1.0em     def encrypt(self, plain):
         \STATE \hskip2.0em	        backend = default\_backend()
         \STATE \hskip2.0em	        padder = padding.PKCS7(128).padder()
         \STATE \hskip2.0em	        plain = padder.update(plain) + padder.finalize()
         \STATE \hskip2.0em	        cipher = Cipher(algorithms.AES(self.key), modes.CBC(self.nonce), backend=backend)
         \STATE \hskip2.0em	        encryptor = cipher.encryptor()
         \STATE \hskip2.0em	        ct = encryptor.update(plain) + encryptor.finalize()
         \STATE \hskip2.0em	        return ct
        \STATE
         \STATE \hskip1.0em     def decrypt(self, ct):
         \STATE \hskip2.0em	        backend = default\_backend()
         \STATE \hskip2.0em	        unpadder = padding.PKCS7(128).unpadder()
         \STATE \hskip2.0em	       cipher = Cipher(algorithms.AES(self.key), modes.CBC(self.nonce), backend=backend)
         \STATE \hskip2.0em	       decryptor = cipher.decryptor()
         \STATE \hskip2.0em	         plain = decryptor.update(ct) + decryptor.finalize()
         \STATE \hskip2.0em	        plain = unpadder.update(plain) + unpadder.finalize()
         \STATE \hskip2.0em	        return plain[4:]
        \STATE
        \STATE \hskip1.0em     def getEncCommand(self, opcode, arguments):
        \STATE \hskip2.0em	        plain\_command = self.allocateCommandCount() + opcode + arguments
        \STATE \hskip2.0em	        return self.encrypt(plain\_command)
        \STATE
        \STATE \hskip1.0em     def getDecCommand(self, ct):
        \STATE \hskip2.0em	        return self.decrypt(ct)
        \STATE
        \STATE \hskip1.0em     def getEncKey(self):
        \STATE \hskip2.0em	        arr = self.encryptionKey + bytes.fromhex("00000001") + self.nonce
        \STATE \hskip2.0em	        digest = hashlib.sha256(arr)
        \STATE \hskip2.0em	        key = digest.hexdigest()
        \STATE \hskip2.0em	        return bytes.fromhex(key)[:16]
        \STATE
        \STATE \hskip1.0em     def allocateCommandCount(self):
        \STATE \hskip2.0em	        return self.cmd\_cnt.to\_bytes(4, byteorder = 'little')
        \STATE
        \STATE myClass = MyClass(encryptionKey, nonce, cmd\_cnt)
        \STATE encrypted\_command = myClass.getEncCommand(opcode,arguments)
        \STATE decrypted\_command = myClass.getDecCommand(encrypted\_command)
    \end{algorithmic}
\end{breakablealgorithm}

\FloatBarrier

==> algorithms/getEncnonce.tex <==
\begin{algorithm}
    \caption{getEncnonce(plain, iv, key)}
    \begin{algorithmic}[1]
        \STATE def getEncnonce(plain, iv, key):     
        \STATE \hskip1.0em	backend = default\_backend()     
        \STATE \hskip1.0em	padder = padding.PKCS7(128).padder()     
        \STATE \hskip1.0em	unpadder = padding.PKCS7(128).unpadder()     
        \STATE \hskip1.0em	plain = padder.update(plain) + padder.finalize()     
        \STATE \hskip1.0em	cipher = Cipher(algorithms.AES(key), modes.CBC(iv), backend=backend)     
        \STATE \hskip1.0em	encryptor = cipher.encryptor()     
        \STATE \hskip1.0em	ct = encryptor.update(plain) + encryptor.finalize()     
        \STATE \hskip1.0em	return ct
    \end{algorithmic}
\end{algorithm}


==> algorithms/getKey.tex <==
\begin{algorithm}
    \caption{getEncnonce(plain, iv, key)}
    \begin{algorithmic}[1]
        \STATE def getKey(mastersecret):     
        \STATE \hskip1.0em	bArr2 = b"bleAuthentication"     
        \STATE \hskip1.0em	bArr3 = bytes.fromhex("00000001")     
        \STATE \hskip1.0em	bArr4 = mastersecret + bArr3 + bArr2     
        \STATE \hskip1.0em	digest = hashlib.sha256(bArr4)     
        \STATE \hskip1.0em	key = digest.hexdigest()     
        \STATE \hskip1.0em	key = bytes.fromhex(key)[:16]     
        \STATE \hskip1.0em	return key
    \end{algorithmic}
\end{algorithm}


==> algorithms/privacyIDPool.tex <==
\begin{algorithm}
    \caption{privacyIDPool generation} 
    \begin{algorithmic}[1]
        \STATE def getPrivacyPool(iv, privacyIdSeed, mastersecret, poolsize):
        \STATE \hskip1.0em	privacyPool = set()
        \STATE \hskip1.0em	for i2 in range(1,poolsize+1):
        \STATE \hskip2.0em		bArr = bytearray(len(privacyIdSeed)+4)
        \STATE \hskip2.0em		b = (i2 >> 8) \& 255         
        \STATE \hskip2.0em		b2 = (i2 \& 255)         
        \STATE \hskip2.0em		bArr[0] = b         
        \STATE \hskip2.0em		bArr[1] = b2         
        \STATE \hskip2.0em		bArr[2:10] = privacyIdSeed         
        \STATE \hskip2.0em		bArr[10] = b         
        \STATE \hskip2.0em		bArr[11] = b2         
        \STATE \hskip2.0em		backend = default\_backend()         		
        \STATE \hskip2.0em		padder = padding.PKCS7(128).padder()         
        \STATE \hskip2.0em		bArr = padder.update(bArr) + padder.finalize()  
        \STATE \hskip2.0em		cipher = Cipher(algorithms.AES(mastersecret),modes.CBC(iv),backend=backend)     
        \STATE \hskip2.0em		encryptor = cipher.encryptor()         
        \STATE \hskip2.0em		ct = encryptor.update(bArr) + encryptor.finalize()
        \STATE \hskip2.0em		ct = ct[:16]              
        \STATE \hskip2.0em		privacyPool.add(ct)     
        \STATE \hskip1.0em	return privacyPool
    \end{algorithmic}
\end{algorithm}



==> figs/advformat.tex <==
\begin{figure}[H]
\centering
  \begin{adjustbox}{width=\textwidth}
\iffalse
    \begin{tabular}{|c|c|c|c|c|c|} 
    \hline
    Byte 0  & Bytes 1-3  & Bytes 4-11 & Byte 12 & Bytes 13-15 & Bytes 16-19  \\ 
    \hline
     \begin{tabular}{@{}c@{}} version \\ adv type \\ tag state\end{tabular}
     & aging counter & privacy ID & 
      \begin{tabular}{@{}c@{}} region ID \\ encryption flag \\ UWB flag \\ battery level\end{tabular}
     & Reserved & Signature \\
    \hline
    \end{tabular}
\fi

\begin{tikzpicture}[font=\ttfamily,
array/.style={matrix of nodes,nodes={draw, minimum size=7mm},column sep=-\pgflinewidth, row sep=0.5mm, nodes in empty cells,
row 1/.style={nodes={draw=none, fill=none, minimum size=5mm}},
row 1 column 2/.style={nodes={draw}},row 1 column 3/.style={nodes={draw}},row 1 column 5/.style={nodes={draw}},row 1 column 6/.style={nodes={draw}}, minimum size=15mm }]
{\setlength{\tabcolsep}{3em}
\matrix[array] (array) {
0 & 1-3 & 4-11 & 12 & 13-15 & 16-19 \\
15 & 6b fa 00 & c8 40 62 b2 8f 00 e2 60 & c3 & 00 00 00 & ad 01 8b 47 \\};
}
%\node[draw, fill=gray!50, minimum size=4mm] at (array-2-1) (box1) {15};


\begin{scope}[on background layer]
\fill[gray!10] (array-1-1.north west) rectangle (array-1-6.south east);
\end{scope}

\draw (array-1-2.north)--++(90:2mm) node [above] (first) {aging counter};

\draw (array-1-3.north)--++(90:2mm) node [above] (first) {privacy ID};
\draw (array-1-5.north)--++(90:3mm) node [above] (first) {reserved};
\draw (array-1-6.north)--++(90:2mm) node [above] (first) {signature};

\node [below=20mm, align=center, anchor=south west] at
(array-2-1.south west) (0) {
\scalebox{.8}{
  {\setlength{\tabcolsep}{.2em}
    \begin{tabular}{|c|c|c|c|} 
        \multicolumn{4}{c}{Byte 0: 0x15} \\
        \hline
        Bit & 0-3 & 4 & 5-7   \\ 
        \hline
         Data & version & adv type & tag state \\ 
         \hline
         Value &  0x01 & 0x00 & 0x05 \\
        \hline
        \end{tabular}
        }
    }
    
};


\node [below=35mm, align=center, anchor=south] at
(array-2-4.south) (12) {
\scalebox{.8}{
  {\setlength{\tabcolsep}{.2em}
    \begin{tabular}{|c|c|c|c|c|} 
        \multicolumn{5}{c}{Byte 12: 0xC3} \\
        \hline
        Bit & 0-3 & 4 & 5 & 6-7   \\ 
        \hline
         Data & region ID & encryption flag & UWB flag & battery level \\ 
         \hline
         Value &  0x0c & 0x00 & 0x00 & 0x03 \\
        \hline
        \end{tabular}
        }
    }
};


\draw (0)--(array-2-1.south);
\draw (12)--(array-2-4.south);

%
\end{tikzpicture}
\end{adjustbox}
\end{figure}


==> fmm.tex <==
\section{Offline Finding protocol for smartphones}
\label{sec:fmm}

In this section, we discuss our findings in the reverse engineering of offline-finding features of the FMM app. The results of this section apply to all versions of FMM app (with the offline finding features) prior to version 7.2.24.12 (July 2022). We have not studied comprehensively the patched FMM app, but some preliminary findings related to how the advertisement payload is generated is given in Appendix~\ref{sec:privID-obf}. 

%\subsection{Find My Mobile in Details}
The OF protocol has multiple modes of operations that depend on the functions supported by the devices involved.
We outline the main OF protocol %that applies to mobile devices, 
which consists of four main operations: Device/Account Registration, Offline (Lost) Device Operation, Online (Helper) Device Operation, and Device/Account Deregistration. 
To simplify presentation, we omit the detailed concrete details of various messages exchanged and would refer to some important data symbolically. We also conflate the different servers used in the OF protocol to a single entity, which we simply refer to as "the server". 

The protocol can be summarised as follows. Initially, devices must complete the registration process the server to obtain various parameters that will be used in the offline operation. When a registered device goes offline, it starts advertising a unique payload that identifies itself. This payload is picked up by nearby online (registered) devices which parse the payload extracting the device’s identifier. The online device then accesses available location services to find out its own location. It then sends the lost device’s identifier and the location through to the server. The owner of the lost device can then access the server to find out its location. Further details of each operation are outlined below.

\subsection{Device/Account Registration}
The Offline Finding (OF) feature can be enabled on Samsung smartphones in the device settings when the device is signed in with a Samsung account. The device will then make an HTTPs request to the \lstinline$/v1/kms/cf/device/registerDevice$ URL of the \lstinline$samsungdive$ server to register itself to the OF network. The request contains the following information:

\begin{itemize}
    \item Secret key: 16-byte random generated by Java Random.
    \item Device ID: Base64 encoding of an MD5 hash of the device’s IMEI, which is constant and unique for a device.
    \item User ID: A value associated with the Samsung account logged in.
    \item Other information such as device type, region code, client version, and device model. 
\end{itemize}

The server then responds with several pieces of information; the most important one (from a security/privacy perspective) is the \lstinline$PrivateIDConfig$, which consists of a 16-byte secret key, an IV (\lstinline$PrivacyIV$), and a size parameter (\lstinline$PrivacyPoolSize$) that will be used to generate BLE advertisements for the OF operations.

The IV value is fixed to the same 16-byte value (i.e., \texttt{"+IABCfvBZHJYFUek8vp3Gg=="} in base64 encoding)  across accounts and devices.
The privacy ID pool size determines the amount of possible advertising values the device will generate. This has also been observed to be standard for all devices, taking the value 51. This means that there are only 51 possible advertisement payloads from a lost device.

\subsection{Offline (Lost) Device Operation}
When an OF registered device no longer has an active network connection, it enters ‘Lost Mode’ and triggers the Offline Finding service to start. The lost device then creates a GATT server profile and starts advertising on the main OF service UUID (FD69). The advertising is the fundamental operation for lost devices as part of the main OF protocol. The GATT server is not directly used by the main OF protocol, however it can be interacted with via BLE and is used as part of secondary OF protocols. 

The GATT profile of a lost device contains two services: the encryption service and the FME service. In our description below, we will refer to these services and their associated characteristics symbolically -- the concrete UUIDs for each of these can be found in Appendix~\ref{sec:fmm-details}. 
\begin{itemize}
\item {\bf Encryption Service}(\texttt{ENCRYPTION}). 
This service is used to implement a challenge-response protocol for authenticating a device that wants to connect to the lost device. It contains three characteristics (see Table~\ref{tbl:char-auth}):
The \texttt{SUPPORTED\_CIPHER} characteristic is readable and contains information about the cipher to be used, which is AES/CBC/PKCS7. The \texttt{NONCE} characteristic is readable and returns an IV to be used during encryption. This IV is a random nonce that is generated using Java \texttt{SecureRandom} each time a client connects to the server. The \texttt{ENONCE} characteristic is writeable and expects to receive an encrypted version of the string ``smartthings”. This string must be encrypted using the given IV and with the device’s secret key (from the \texttt{PrivateIDConfig}). Writing the correct ciphertext to the encrypted nonce characteristic completes the handshake between client and server.

\item {\bf FME Service} (\texttt{FME}). 
    After completing the handshake, the client is now authenticated and can interact with the characteristics in the FME service. The device’s alarm can be set to ring by writing the byte 01 (encrypted using the same cipher) to the \texttt{ALARM} characteristic (UUID 4a1351bb-d617-4612-a8e3-8dee6ca13e7b).

\end{itemize}


\paragraph{Lost Mode Advertising.}
The lost mode advertisements are the fundamental part of the OF protocol. The lost device generates an advertisement containing a unique identifying payload which is picked up by a helper and reported to Samsung. A key component of the advertisement payload is the {\em privacy ID} that identifies the device uniquely. A device can generate a number of privacy IDs, depending on the privacy ID pool parameter in \texttt{PrivateIDConfig}. 

Let $k$, $iv$ and $p$ denote, respectively, the secret key, IV and the privacy ID pool from the device’s \texttt{PrivateIDConfig}. To generate a privacy ID, first we compute a 20-byte array: 
\[
x_i = \mbox{
    \resizebox{.8\columnwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|} 
    \hline
    Byte 0 & Byte 1 & Bytes 2-17 & Byte 18 & Byte 19         \\ 
    \hline
    00 & $i$ & $k$ & 00 & $i$ \\
    \hline
    \end{tabular}
    }
}
\]
where $i$ is a 1-byte random nonce in $\{1, \dots, p\}$, i.e., it is a random 1-byte value bounded by the privacy ID pool. From $x_i$, one then generates a ciphertext: 
\[
y_i = E_{k}(iv, x_i)
\]
where $E$ denotes the AES/CBC/PKCS7 cipher, initialized with the key $k$ and the initialization vector $iv.$ 
The privacy ID corresponding to each $i$ is then computed by taking the first 12 bytes of $y_i$: 
\[ 
pid_i = y_i[0:11]. 
\]

Finally, the advertisement payload is generated from the privacy ID combined with various meta data. Table \ref{fig:fmmadv} describes the full advertisement payload.

\definecolor{Gray}{gray}{0.85}
\newcolumntype{a}{>{\columncolor{Gray}}c}
\begin{table}[htp]
    \centering
    \caption{FMM Lost Mode Advertisement Structure}
    \label{fig:fmmadv}

    \resizebox{.8\columnwidth}{!}{%
    \begin{tabular}{|c|ccc|} 
    \hline
    Byte & 0  & 1-12  & 13 \\ 
    \hline
    Info & operation mode & privacy ID & support info \\ 
    \hline
    \end{tabular}
    }
\end{table}

The first byte describes the operation mode of the OF protocol that is being used by a lost device. In the main OF protocol, this byte is always zero. The last byte contains information about the device’s region and functionalities supported. This last byte varies depending on the device but stays consistent for all advertisements for a device. If two lost mode devices are advertising in the same area, then this last byte can be used as a quasi-differentiator between the two, provided they do not have the same settings/support.

Once the advertising data has been generated, the lost device starts advertising over BLE on the OF service’s UUID FD69. The device will continuously advertise the same data until a timer is triggered that causes it to shuffle the advertising data. This timer is set to trigger every 60 minutes, after which the device generates a new random nonce to be used to generate the advertising data. Since, there are only 51 possible values for the nonce $i$, and it is the only source of non-determinism, there are also only 51 possible values of the advertising data (for a \texttt{PrivateIDConfig}). The lost device repeats this process until it is online again. If an adversary has access to the device’s secret key and IV, then it is trivial to generate the 51 possible values. 



==> gattprofile.tex <==

\begin{figure*}
\centering
\scalebox{.7}{

\begin{tikzpicture}[align=center,>=latex',font=\sffamily]
\tikzstyle{NormalGATT} = [draw=black,thick,rectangle,minimum width=160mm,minimum height=144mm]
\tikzstyle{NormalCHAR} = [draw=black,thick,rectangle,minimum width=72mm,minimum height=15mm]
\tikzstyle{NormalSERV} = [draw=black,thick,rectangle,minimum width=76mm,minimum height=57mm]
\node[label=above:GATT Profile,NormalGATT](GATTProfile){};

\node[label=above:Onboarding Service\\FD59, above right=6mm and 3mm of GATTProfile.south west,anchor=south west,NormalSERV](Onboarding){};
\node[below right=3mm and 2mm of Onboarding.north west,anchor=north west,NormalCHAR](MAC){MAC\_CHAR (read)\\08A11E38-1C6D-4929-9C32-4F32A64985CE};
\node[below=18mm of MAC.north,anchor=north,NormalCHAR](HASH){HASH\_CHAR (read)\\6AC16DB1-F442-4BF4-B804-04C32356465D};
\node[below=18mm of HASH.north,anchor=north,NormalCHAR](FD59CHARS){......};

\node[label=above:Authentication Service\\EEDD5E73-6AA8-4673-8219-398A489DA87C, below right=11mm and 3mm of GATTProfile.north west,anchor=north west,NormalSERV](AUTH){};
\node[below right=3mm and 2mm of AUTH.north west,anchor=north west,NormalCHAR](NONCE){NONCE\_CHAR (indicate, read, write)\\A12BE31C-5B38-4773-9B9D-3D5735233A7C};
\node[below=18mm of NONCE.north,anchor=north,NormalCHAR](ENONCE){ENONCE\_CHAR (indicate, write) \\4EBE81F6-B952-465E-9ECE-5CA39D4E8955};
\node[below=18mm of ENONCE.north,anchor=north,NormalCHAR](CIPHER){CIPHER\_CHAR (read, write)\\50F98BFD-158C-4EFA-ADD4-0A70C2F5DF5D};

\node[label=above:DFU Service\\FE59, below left=11mm and 3mm of GATTProfile.north east,anchor=north east,NormalSERV](DFU){};
\node[below right=3mm and 2mm of DFU.north west,anchor=north west,NormalCHAR,minimum height=50mm](BUTTONLESSDFU){DFU\_CHAR (indicate, write)\\8EC90003-F315-4F60-9FB8-838830DAEA50};

\node[label=above:Command Service\\FD5A, above left=6mm and 3mm of GATTProfile.south east,anchor=south east,NormalSERV](Command){};
\node[below right=3mm and 2mm of Command.north west,anchor=north west,NormalCHAR](ALARM){OWNER\_ALARM\_CHAR\\(indicate, read, write)\\DEE30001-182D-5496-B1AD-14F216324184};
\node[below=18mm of ALARM.north,anchor=north,NormalCHAR](FIRMWARE){FIRMWARE\_CHAR \\(indicate, read, write no response)\\DEE3000C-182D-5496-B1AD-14F216324184};
\node[below=18mm of FIRMWARE.north,anchor=north,NormalCHAR](FD5ACHARS){......};
\end{tikzpicture}
}
\caption{The GATT Server Profile for SmartTags}
\label{table:gatt}
\end{figure*}


==> resources/commands.tex <==

\begin{lstlisting}
{
 "name": "setMaxAllowedBLEConnections",
 "gatt": {
    "service": 
    "0000FD5A-0000-1000-8000-00805F9B34FB",
    "characteristic": "DEE3000D-182D-5496-B1AD-14F216324184",
    "cipher": "aes-cbc-128-pkcs7padding",
    "opCode": "0",
    "arguments": [
    {
        "name": "maxAllowedBLEConnections",
        "value": {
            "valueType": "uint8",
            "min": 1,
            "max": 2
        }
    }
    ]
 }
}
\end{lstlisting}

==> tables/adversarymodel.tex <==
\begin{table}[htp]
  \centering
  \label{tbl:adversary-model}
    \caption{Adversary model}
  \scalebox{0.8}{
{\small %
    \begin{tabular}{p{.3\textwidth}p{.3\textwidth}p{.3\textwidth}p{.3\textwidth}}
      \toprule
      Model & Assumptions & Goals & Capabilities \\
      \midrule
      Proximity-based (A1) &
        (1) within BLE communication range \newline
        (2) control one or more Bluetooth transceivers to cover a larger range &
        (1) Locate a lost device \newline
        (2) Identify and track lost devices for a long period of time despite the payload/mac rotation \newline
        (3) The replayed advertisement data being picked up by a finder device, which result in fake location report being uploaded to the server \newline
        (4) Disable a device over the air &
        (1) Capture devices BLE advertisement data. \newline
        (2) Interact with a device’s GATT server, read/write characteristics \newline 
        (3) Record and replay advertisements. \newline
        (4) Create new advertisements \\
    Network-based (A2) &
        (1) MitM position between the remote server and finder devices. \newline
        (2) MitM position between the remote server and owner devices. &
        (1) Access location of reported lost devices \newline
        (2) Identify finder devices \newline
        (3) Identify lost devices &
        (1) Redirect traffic to a different host. \newline
        (2) Read, intercept, redirect,or modify traffic \\
    Service Operator (A3) &
        (1) Apple/Samsung/Tile as the service provider. \newline
        (2) Controls the OF server infrastructure. &
        (1) Locate individuals and their lost devices. \newline 
        (2) Correlate locations to create a social graph &
        (1) Access to all encrypted location reports and sensitive data. \newline
        (2) Add, remove, or modify reports. \\
    Physical Access (A4) &
        (1) Has direct contact with a victim.  \newline 
        (2) Controls one or more BLE transceivers which may cover a large area. &
        (1) Locate individuals and their lost devices.  \newline 
        (2) Correlate locations to create a social graph &
        (1) Hide a tracker device in the victim’s bag/other belongs \\
    Impersonation (A5) &
        (1) Access to a legitimate tracker device/account. \newline 
        (2) Has access to one or more ESP32 (or similar) systems. \newline 
        (3) Access to Apple, Samsung, Tile’s mobile application or firmware &
        (1) create a more stealthy and powerful tracking device that uses the Apple, Samsung, Tile’s offline finding network for crowd-sourced tracking &
        (1) Record and replay advertisements. \newline 
        (2) Generate new advertisements. \newline 
        (3) Uncover then utilize the encryption algorithms or other important algorithms used by Apple/Samsung/Tile via analysis of the corresponding software/firmware \\
& & & \\
      \bottomrule
    \end{tabular}%
%\vspace{-4mm}
}%
}
\end{table}


==> tables/bleauthentication.tex <==
\begin{table}
\centering
\caption{Input for the SHA-256 digest function (BLE Authentication)}
\begin{tabular}{|c|c|c|} 
\hline
Bytes 0-15    & Byte 16-19                & Bytes 20-53         \\ 
\hline
Master Secret & {00000001} & ``bleAuthentication"  \\
\hline
\end{tabular}
\end{table}


==> tables/commandencryption.tex <==
\begin{table}
\centering
\caption{Input for the SHA-256 digest function (GATT commands)}
\begin{tabular}{|c|c|c|c|c|c|} 
\hline
Bytes 0-15    & Byte 16                & Byte 17                & Byte 18                & Byte 19 & Bytes 20-35         \\ 
\hline
Master Secret & \multicolumn{4}{c|}{00000001} & IV  \\
\hline
\end{tabular}
\end{table}


==> tables/fmm.tex <==
\begin{table}
\centering
\caption{Byte Array Encrypted During Lost Mode Advertising Data Generation}
\begin{tabular}{|c|c|c|c|c|} 
\hline
Byte 0 & Byte 1 & Bytes 2-17 & Byte 18 & Byte 19         \\ 
\hline
00 & $i$ & secret key & 00 & $i$ \\
\hline
\end{tabular}
\end{table}


==> tables/fwdata.tex <==
\begin{table}[htp]
  \centering
    \caption{Format of the transferFirmwareData command}
  \label{table:fwinfo}
    \begin{tabular}{*{3}{cll}}
      \toprule
      Opcode & Argument & Type\\
      \midrule
      \multirow{4}{*}{0x01} 
                & offset & uint32 \\
                &  segmentedFirmwareDataLength & uint16 \\
                &  segmentedFirmwareData &  byteArray \\
                &  argumentsCRC16 & uint8 \\
      \bottomrule
    \end{tabular}
\end{table}


==> tables/fwinfo.tex <==
\iffalse
\vskip -0.8cm
\begin{table}[htp]
  \centering
    \caption{Arguments for the transferFirmwareInformation command}
  \label{table:fwinfo}
    \begin{tabular}{lll}
      \toprule
      Argument & Type & Value (firmware 1.02.06) \\
      \midrule
      totalFirmwareSize & uint32 & 179620 \\
      totalFirmwareCRC16 & uint16 & 37858\\
      newFirmwareVersionLength &  uint8 & 7\\
        newFirmwareVersion  & string & ``1.02.06"\\
        transferWindow & uint8 & 10 \\
      \bottomrule
    \end{tabular}
\end{table}
\fi

\begin{table}[htp]
  \centering
    \caption{Format of the transferFirmwareInformation command}
  \label{table:fwinfo}
    \begin{tabular}{*{3}{cll}}
      \toprule
      Opcode & Argument & Type\\
      \midrule
      \multirow{5}{*}{0x00} 
                & totalFirmwareSize & uint32 \\
                &  totalFirmwareCRC16 & uint16 \\
                &  newFirmwareVersionLength &  uint8 \\
                &  newFirmwareVersion & string \\
                & transferWindow & uint8\\
      \bottomrule
    \end{tabular}
\end{table}


==> tables/gattcommand.tex <==
\begin{table}[H]
\centering
\caption{The structure of a GATT command}
\begin{tabular}{|c|c|c|} 
\hline
Bytes 0-3 & Byte 4  & Bytes 5-N         \\ 
\hline
Command Counter & Command Opcode & Arguments  \\
\hline
\end{tabular}
\end{table}


==> tables/nonceexchange.tex <==
\vskip -0.8cm
\begin{table}[htp]
    \centering
            \caption{Nonce Exchange Observed}

    \label{tbl:nonces}
        \begin{tabular}{ccccc}
          \toprule
          Step & Source & Dest & Data & Description \\
          \midrule
            1 & phone & tag & f596167d22b3b9d6e7f2f23f813b8605 & nonce \\
            2 & tag & phone & db4249bdb224e8c44106d3b5cc2f512b & nonce \\
            3 & phone & tag & f0a6069d49692f81510a244e8ab9e753 & encrypted nonce \\
            4 & tag & phone & f0c1997691d4f334448bbf46643af179 & encrypted nonce \\
          \bottomrule
        \end{tabular}
\end{table}


==> tables/nonregisteredtagadv.tex <==

\begin{table}[htp]
  \centering
    \caption{Format of a non-registered SmartTag's advertisement}
  \label{tbl:smarttag-ads}
    \begin{tabular}{ll}
      \toprule
      Byte(s) & Description \\
      \midrule
        0 & 0x01  \\
        1-4 & mnId, different for each tag\\
        5-7 & setupId \\
        8 & 0x01 \\
        9 & 0x05  \\
        10 & 0x01 \\
        11-13 & \specialcell{The last two bytes of the MAC address\\ e.g., 33444431 if the MAC address ends with 3D:D1 } \\
      \bottomrule
    \end{tabular}
\end{table}


==> tables/privacyID.tex <==
\begin{table}
\centering
\caption{Input for the SHA-256 digest function (Privacy IDs)}
\begin{tabular}{|c|c|c|} 
\hline
Bytes 0-15    & Byte 16-19 & Bytes 20-33         \\ 
\hline
Master Secret & {00000001} & ``privacy"  \\
\hline
\end{tabular}
\end{table}


==> tables/privacyidplaintext.tex <==
\begin{table}
\centering
\caption{Input data for the AES algorithm (Privacy IDs)}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|} 
\hline
Byte 0  & Byte 1  & Bytes 2-9 & Byte 10 & Byte 11  \\ 
\hline
${i\gg 8}\land 256$ & $i\land 256$ & Privacy ID seed & $(i\gg 8)\land 256$ & $i\land 256$ \\
\hline
\end{tabular}}
\end{table}


==> tables/signing.tex <==
\begin{table}
\centering
\caption{Input for the SHA-256 digest function (Signature)}
\begin{tabular}{|c|c|c|} 
\hline
Bytes 0-15    & Bytes 16-19 & Bytes 20-33         \\ 
\hline
Master Secret & 00000001 & ``signing"  \\
\hline
\end{tabular}
\end{table}


==> tables/verification.tex <==
\begin{table}[htp]
  \centering
  
        \caption{characteristics read by the phone during the verification step}
  \label{tbl:chars}
    \begin{tabular}{lll}
      \toprule
       Characteristics & Description & value\\
      \midrule
        6ac16db1f4424bf4b80404c32356465d & serial number hash (32 bytes) & Different for each tag \\
        5352fee4f3bc462cba7c279873bcdd71 & model name & EI-T5300 \\
        5b5f7a4c257e484192d50042658122b6 & cipher & AES\_128-CBC-PKCS7Padding \\
      \bottomrule
    \end{tabular}
\end{table}

